Ohm-GPU: Integrating New Optical Network and Heterogeneous Memory into GPU Multi-Processors

Traditional graphics processing units (GPUs) suffer from the low memory capacity and demand for high memory bandwidth. To address these challenges, we propose Ohm-GPU, a new optical network based heterogeneous memory design for GPUs. Specifically, Ohm-GPU can expand the memory capacity by combing a set of high-density 3D XPoint and DRAM modules as heterogeneous memory. To prevent memory channels from throttling throughput of GPU memory system, Ohm-GPU replaces the electrical lanes in the traditional memory channel with a high-performance optical network. However, the hybrid memory can introduce frequent data migrations between DRAM and 3D XPoint, which can unfortunately occupy the memory channel and increase the optical network traffic. To prevent the intensive data migrations from blocking normal memory services, Ohm-GPU revises the existing memory controller and designs a new optical network infrastructure, which enables the memory channel to serve the data migrations and memory requests, in parallel. Our evaluation results reveal that Ohm-GPU can improve the performance by 181% and 27%, compared to a DRAM-based GPU memory system and the baseline optical network based heterogeneous memory system, respectively.

==> introduction-old.tex <==
Traditional memory systems face great challenges to satisfy the increasing data bandwidth demands from the emerging data-hungry applications such as artificial intelligence and cloud computing \cite{memorywall1, memorywall2, gai2016cost}. 
In contrast to the processor whose performance can be improved by integrating more transistors, the bandwidth of off-chip memory is not scalable, due to the area and power overhead of the electrical transceivers and the limit number of I/O pins in package interconnects. Optical network, which is built from CMOS-compatible integrated silicon-photonic technology \cite{shacham2007design, beausoleil2008nanoelectronic}, has been widely evaluated in both academy and industry to replace the existing electrical interconnects in memory systems \cite{li2013exploring, beamer2010re, wen2016silicon, udipi2011combining}. Compared to the electrical memory channel, the dense wavelength-division multiplexing (DWDM) technique in the optical network allows different wavelengths in a single waveguide to carry multiple data streams, which can deliver two orders of magnitude higher bandwidth.

The optical network proposed in prior work is typically deployed in DRAM/PRAM-only memory system as a memory channel. Such design is well optimized to provide point-to-point communication between the memory controller and the memory packages. Nevertheless, the introduction of the Optane DC persistent memory module (PMM) significantly changes the architecture of memory system \cite{optaneDC}, making the prior optical network sub-optimal to deliver high memory bandwidth. Optane DC PMM is a new type of dual inline memory module (DIMM), whose storage medium is made from the emerging non-volatile memory. While Optane DC PMM can provide 8$\times$ higher capacity than traditional DRAM-based DIMM \cite{optane-size} and ensure data persistency, its read and write bandwidths are 4$\times$ and 6$\times$ slower than those of DRAM, respectively \cite{optane-perf}. Therefore, to balance the capacity and performance, the common practice is to group Optane DC PMM with DRAM as a heterogeneous memory. Unlike DRAM/PRAM-only memory system, the new heterogeneous memory is mainly organized to support three working scenarios: 1) DRAM is accessed as main memory and Optane DC PMM backs up the data of DRAM as persistent storage (system persistency scenario) \cite{narayanan2012whole, kateja2017viyojit}; 2) both DRAM and Optane DC PMM work as planar memory, which are accessed by unified address space (planar memory scenario) \cite{shin2012adaptive, dhiman2009pdram}; 3) PRAM works as main memory and DRAM is an inclusive cache of PRAM (two-level memory scenario) \cite{park2018bibim}. In addition to serving the memory requests from the user applications, the system persistency scenario and the two-level memory scenario also migrate data between DRAM and Optane DC PMM. Specifically, the system persistency scenario needs to periodically copy the modified pages in DRAM to Optane DC PMM for data persistency, while the two-level memory scenario fetches data from Optane DC PMM to DRAM for every cache miss in DRAM. Although planar memory scenario does not require data migration, moving hot pages from slow memory devices (Optane DC PMM) to fast memory device (DRAM) can effectively reduce memory access latency, which turns out better system performance \cite{wang2016duang}. 

\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{figs/motiv_fig.eps}
	\vspace{-15pt}
	\caption{\label{fig:motiv1}Memory bandwidth analysis for user application and data migration.\vspace{-15pt}}
	\vspace{-5pt}
\end{figure}

Unfortunately, the data migration between DRAM and Optane DC PMM consumes the limited memory bandwidth, which is not negligible. We implement traditional optical network \cite{li2013exploring} in the three scenarios, and collect the effective memory bandwidth consumed by user applications and the wasted memory bandwidth used for data migration in various workloads \cite{nalli2017analysis, henningstandard}. Figure \ref{fig:motiv1} shows the fraction of effective and wasted memory bandwidths. As shown in the figure, the wasted bandwidth, on average, accounts for 33\%, 29\%, and 45\% of total bandwidth in system persistency scenario, planar memory scenario and two-level memory scenario, respectively. This is because, while memory requests are served in 64B access granularity, data migration requires moving the whole 4KB pages via the memory channel. In addition, as the memory communication protocol does not allow direct DIMM-to-DIMM communication, the target data needs moving from the source DIMM to the memory controller first and then moving back from the memory controller to the destination DIMM, which double the cost of bandwidth usage.

\begin{figure*}
	\centering
	\includegraphics[width=1\linewidth]{figs/motiv.eps}
	\vspace{-15pt}
	\caption{\label{fig:motiv}The data movement in heterogeneous memory.\vspace{-15pt}}
	\vspace{-5pt}
\end{figure*}

To mitigate the impact of data migration on memory bandwidth, prior work propose to do the data migration at background \cite{shin2012adaptive, wang2016duang}. This solution requires a good prediction method, which can accurately find out the idle time slots of memory channel in near future. However, the implementation of idle time predictor in OS-level or hardware is non-trivial. In addition, data migration cannot benefit from the predictor, when it has to be prioritized to avoid blocking the whole system (e.g., when the number of dirty pages is higher than the threshold set by the battery budget in system persistency scenario or there is DRAM cache read miss in two-level memory scenario). 

Instead, the photonic-based memory channel can be architected to minimize the bandwidth overhead of data migration. Specifically, in addition to serving the memory requests in the main data path between the memory controller and DIMMs, optical network is able to simultaneously set up one more data path to do the data transfer, which can benefit the data migration. The extra data path is called as \emph{phantom} path. Specifically, when a transmitter sends data to its receiver, the phantom path can broadcast the same data stream to any other receiver. Nevertheless, the phantom path is able to transfer new data stream between a new couple of transmitter and receiver, only if the phantom path does not overlap with the main data path. 

In this work, we propose PHANTOM, a new optical network design for heterogeneous memory system, which can fully leverage the phantom path to mitigate the impact of data migration on memory bandwidth. Specifically, we build a new optical network infrastructure to enable phantom path in the optical waveguide. This infrastructure is optimized to minimize the routine conflicts between main data path and phantom path with minor area cost and low power consumption. We further integrate optical configuration module in memory controller to arbitrate whether turn on or turn off the phantom path. In addition, we propose a new phantom path aware scheduling policy in memory controller, which selectively choose a pair of memory requests to schedule in the main data path and the phantom path for better parallelism. By leverging the proposed optical network based memory system, we optimize the three working scenarios of heterogeneous memory to hide the penalty of data migration, which is shown in Figure \ref{fig:motiv}. As shown in the figure, for system persistency scenario, when user application accesses the modified pages in DRAM, We propose to opportunisitically broadcast the same pages to Optane DC PMM via the phantom path, so that we can reduce the number of pages for backup in future. For planar memory scenario, we propose to directly migrate data between DRAM and Optane DC PMM in the phantom path. This operation does not occupy the memory channel, as it can be issued in parallel with other memory requests. For two-level memory scenario, when there is DRAM cache miss, the Optane DC PMM can broadcast the target data block to both DRAM and user application. The remaining data blocks in the accessed page can be directly migrated from DRAM to Optane DC PMM via the phantom path. To sum up, compared to the traditional photonic-based memory system, our evaluation results show that PHANTOM can improve the memory bandwidth utilization by XX\%, XX\% and XX\%, respectively, in system persistency scenario, planar memory scenario and two-level memory scenario. 


%Our main contributions can be summarized as follows.

%New photonic infrastructure to enable phantom path.

%Phantom path aware memory controller.

%Customized optimization for heterogeneous memory system.
